Formal Verification of Consistency for Systems with Redundant Controllers

A potential problem that may arise in the domain of distributed control systems is the existence of more than one primary controller in redundancy plans that may lead to inconsistency. An algorithm called NRP FD is proposed to solve this issue by prioritizing consistency over availability. In this paper, we demonstrate how by using modeling and formal verification, we discovered an issue in NRP FD where we may have two primary controllers at the same time. We then provide a solution to mitigate the identified issue, thereby enhancing the robustness and reliability of such systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{169}
\providecommand{\publicationstatus}{F. Lang, M. Volk (Eds):\\
Models for Formal Analysis of Real Systems (MARS 2024)\\
EPTCS 399, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.399.8}{10.4204/EPTCS.399.8}}
\pdfoutput=1

